Z-Forcing: Training Stochastic Recurrent Networks

Many efforts have been devoted to training generative latent variable models with autoregressive decoders, such as recurrent neural networks (RNN). Stochastic recurrent models have been successful in capturing the variability observed in natural sequential data such as speech. We unify successful ideas from recently proposed architectures into a stochastic recurrent model: each step in the sequence is associated with a latent variable that is used to condition the recurrent dynamics for future steps. Training is performed with amortized variational inference where the approximate posterior is augmented with a RNN that runs backward through the sequence. In addition to maximizing the variational lower bound, we ease training of the latent variables by adding an auxiliary cost which forces them to reconstruct the state of the backward recurrent network. This provides the latent variables with a task-independent objective that enhances the performance of the overall model. We found this strategy to perform better than alternative approaches such as KL annealing. Although being conceptually simple, our model achieves state-of-the-art results on standard speech benchmarks such as TIMIT and Blizzard and competitive performance on sequential MNIST. Finally, we apply our model to language modeling on the IMDB dataset where the auxiliary cost helps in learning interpretable latent variables. Source Code: \url{https://github.com/anirudh9119/zforcing_nips17}

==> misc.tex <==
\begin{table}[t]
\small
\begin{center}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Models} & BLIZZARD & TIMIT \\
   	\midrule
    RNN-Gauss & 3539 & -1900 \\
    RNN-GMM & 7413 & 26643 \\
    VRNN-I-Gauss~\citep{vrnn} & $\ge$ 8933 & $\ge$ 28340 \\ 
    VRNN-Gauss~\citep{vrnn} & $\ge$ 9223 & $\ge$ 28805 \\
    VRNN-GMM~\citep{vrnn} & $\ge$ 9392 & $\ge$ 28982 \\
    SRNN~\citep{srnn} & $\ge$ 11991 & $\ge$ 60550 \\
    \midrule
    Ours & $\ge$13048 & $\ge$ 68351 \\
    Ours + aux & $\ge$ \textbf{14315} & $\ge$ \textbf{70751} \\
    \midrule
    *Ours (2048 units) & $\ge$ 16933 & - \\
    *Ours + aux (2048 units) & $\ge$ \textbf{17048} & - \\
    \bottomrule
  \end{tabular}
\end{center}
\caption{\label{tab:nll_speech} Average log-likelihood per sequence on the test sets on the BLIZZARD and TIMIT datasets. The line ``Ours + aux'' denotes our model trained with the auxiliary cost, while for ``Ours'' we set $\lambda_{\textrm{aux}} = 0$. Models denoted by * have twice the capacity in their $f_{\cdot}$ networks.
}
\end{table}




\begin{table}[t]
\small
\begin{center}
  \begin{tabular}{lc}
    \toprule
    \textbf{Models} & MNIST NLL\\
   	\midrule
    DBN 2hl~\citep{germain2015made}&     $\approx$ 84.55 \\
	NADE~\citep{uria2016neural}  &      88.33 \\
    EoNADE-5 2hl~\citep{raiko-nips2014} &     84.68 \\
    DLGM 8 leapfrog steps~\citep{salimans2014markov}       &       $\approx$ 85.51 \\
    DARN 1hl~\citep{gregor2015draw}	&     $\approx$ 84.13 \\
    DRAW~\citep{gregor2015draw}        &      $\leq$ 80.97 \\
    PixelVAE ~\citep{gulrajani2016pixelvae} & $\le$ 80.64 \\
    PixelVAE (gated)~\citep{gulrajani2016pixelvae} & $\approx$ \textbf{79.02}$^\blacktriangledown$  \\
    Professor Forcing~\citep{goyal+lamb+al-2016-nips}  & 79.58$^\blacktriangledown$ \\
    PixelRNN (1-layer)~\citep{oord2016pixel}           & 80.75 \\
    PixelRNN (7-layer)~\citep{oord2016pixel}           & 79.20$^\blacktriangledown$ \\
    \midrule
    Ours + aux & $\le$ 80.42 \\
    \bottomrule
  \end{tabular}
\end{center}
\caption{\label{tab:nll_mnist} Test set negative log-likelihood for sequential MNIST. $^\blacktriangledown$ denotes lower performance of our model with respect to the baselines.}
\end{table}


